Real-Time Model Predictive Control of Vehicles with Convex-Polygon-Aware Collision Avoidance in Tight Spaces

This paper proposes vehicle motion planning methods with obstacle avoidance in tight spaces by incorporating polygonal approximations of both the vehicle and obstacles into a model predictive control (MPC) framework. Representing these shapes is crucial for navigation in tight spaces to ensure accurate collision detection. However, incorporating polygonal approximations leads to disjunctive OR constraints in the MPC formulation, which require a mixed integer programming and cause significant computational cost. To overcome this, we propose two different collision-avoidance constraints that reformulate the disjunctive OR constraints as tractable conjunctive AND constraints: (1) a Support Vector Machine (SVM)-based formulation that recasts collision avoidance as a SVM optimization problem, and (2) a Minimum Signed Distance to Edges (MSDE) formulation that leverages minimum signed-distance metrics. We validate both methods through extensive simulations, including tight-space parking scenarios and varied-shape obstacle courses, as well as hardware experiments on an RC-car platform. Our results demonstrate that the SVM-based approach achieves superior navigation accuracy in constrained environments; the MSDE approach, by contrast, runs in real time with only a modest reduction in collision-avoidance performance.

==> src/acknowledgement.tex <==
\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

==> src/note <==

\begin{comment}
  The position of vehicle's vertices $\bm{p}_{\mathrm{car},i}^{\mathrm{vertex}}\in\mathbb{R}^2 (i\in\{1,2,3,4\})$ are calculated as follows:
  \begin{align}
    \bm{p}_{\mathrm{car},i}^{\mathrm{vertex}}=
    \begin{bmatrix}
      \cos\theta &-\sin\theta\\
      \sin\theta & \cos\theta
    \end{bmatrix}\ ^{\mathrm{o}}\bm{p}_{\mathrm{car},i}^{\mathrm{vertex}} \label{eq:rotated_car_vertex},
  \end{align}
  where $^{\mathrm{o}}\bm{p}_{\mathrm{car},i}^{\mathrm{vertex}}$ is a relative position of the vertex $i$ from the vehicle's position $\bm{p}_{\mathrm{car}}$ at its yaw angle $\theta=0$, and given by following equations:
  \honda{この式に$p_{\rm{car}}$が入っていないのはおかしいのでは？}
  \begin{align}
    &^{\mathrm{o}}\bm{p}_{\mathrm{car},1}^{\mathrm{vertex}} = 
    \begin{pmatrix} 
      -l_{\mathrm{roh}}-d_{\mathrm{margin}} \\  w_{\mathrm{car}}/2+d_{\mathrm{margin}} 
    \end{pmatrix} 
    \label{eq:default_car_vertex1}\\
    &^{\mathrm{o}}\bm{p}_{\mathrm{car},2}^{\mathrm{vertex}} = 
    \begin{pmatrix} 
      -l_{\mathrm{roh}}-d_{\mathrm{margin}} \\ -w_{\mathrm{car}}/2-d_{\mathrm{margin}}
    \end{pmatrix} 
    \label{eq:default_car_vertex2}\\
    &^{\mathrm{o}}\bm{p}_{\mathrm{car},3}^{\mathrm{vertex}} = 
    \begin{pmatrix} 
      l_{\mathrm{car}}-l_{\mathrm{roh}}+d_{\mathrm{margin}} \\ -w_{\mathrm{car}}/2-d_{\mathrm{margin}} 
    \end{pmatrix} 
    \label{eq:default_car_vertex3}\\
    &^{\mathrm{o}}\bm{p}_{\mathrm{car},4}^{\mathrm{vertex}} = 
    \begin{pmatrix} 
      l_{\mathrm{car}}-l_{\mathrm{roh}}+d_{\mathrm{margin}} \\ w_{\mathrm{car}}/2+d_{\mathrm{margin}}
    \end{pmatrix} 
    \label{eq:default_car_vertex4}
  \end{align}
  where $l_{\mathrm{car}}, w_{\mathrm{car}}, l_{\mathrm{roh}}, d_{\mathrm{margin}}$ are the vehicle's length, width, rear overhang and margin, respectively.
  To avoid getting too close to obstacles, the vehicle's shape is considered as a rectangle stretched $d_{\mathrm{margin}}$ longitudinally and laterally from its actual one.
\end{comment}

\section{Experiments}

\subsection{Simulation Settings}

In simulations, we compare the avoidance methods above in terms of the calculation cost and ability to navigate.
The scenarios are reverse parking, parallel parking, and avoidance of obstacles with various shapes in tight spaces.
With referring to Japanese standard vehicles, we set the vehicle's length $l_{\mathrm{car}}=4.0\ \mathrm{m}$, width $w_{\mathrm{car}}=1.7\ \mathrm{m}$, wheelbase $l_{\mathrm{f}}=2.5\ \mathrm{m}$, rear overhang $l_{\mathrm{roh}}=0.8\ \mathrm{m}$ and margin $d_{\mathrm{margin}}=0.05\ \mathrm{m}$.
In addition, we set the vehicle's absolute limit of velocity $v_{\mathrm{lim}}=2\ \mathrm{m/s}$, steering angle $\delta_{\mathrm{lim}}=0.70\ \mathrm{rad}$, acceleration $\dot{v}_{\mathrm{lim}}=1\ \mathrm{m/s^2}$, and steering angle velocity $\dot{\delta}_{\mathrm{lim}}=6.28\ \mathrm{rad/s}$.
The other vehicle's states have no constraints.
All simulations were done on a notebook with Intel Core i7-1165G7 CPU @ 2.80GHz x 4 processors and 16GB of memory.
\begin{figure}[t]
  \begin{minipage}[t]{0.45\hsize}
  \centering
  \includegraphics[width=7cm]{fig/reverse_parking/init_pos.pdf}
\end{minipage}\\
\begin{minipage}[t]{0.45\hsize}
  \centering
  \includegraphics[width=8cm]{fig/parallel_parking/init_pos.pdf}
\end{minipage}
  \caption{Environments of reverse parking (Above) and parallel parking (Below).}
  \label{fig:environment}
\end{figure}
\figref{fig:environment} shows the environments of reverse and parallel parking.
There are some vehicles parked before the ego vehicle parks, and it is going to park among them.
105 and 66 blue points placed $0.5\ \mathrm{m}$ and $0.2\ \mathrm{m}$ apart are initial positions in reverse and parallel parking, respectively.
All initial vehicle states except the initial position are zero, and tasks are parking in red parking spots.

\subsection{Implementation Details}

\honda{移植中}
In simulations, time intervals of the prediction horizon $\Delta\tau$ and control cycles $\Delta t$ are the same as 0.2 s.
In experiments, time intervals of the prediction horizon $\Delta\tau$ are not changed. 
However, each of the control cycles $\Delta t$ is the same as the solving time $t_s$ at time $t$ because control inputs are given by the solution of the optimal control problem. In addition, the solving time $t_s$ is generally shorter than time intervals of the prediction horizon $\Delta\tau$. Thus, control cycles $\Delta t$ can be shortened in order to deal with changes in the situation and errors in dynamics.

\begin{table}[t]
  \centering
	\footnotesize
  \caption{Weight Parameters in the Cost Function}
  \label{tab:parameter}
	\begin{tabular}{|r|r|r|}\hline
    & reverse parking & parallel parking\\\hline
		$S_{\mathrm{f}}$ & $\mathrm{diag}[300,300,15,600,15]$ & $\mathrm{diag}[800,800,20,400,20]$ \\
		$Q$ & $\mathrm{diag}[0.25,0.25,0.05,1,0.05]$ & $\mathrm{diag}[0.5,0.5,0.05,0.5,0.05]$ \\ 
		$R$ & $\mathrm{diag}[0.2,20]$ & $\mathrm{diag}[0.2,20]$ \\ \hline
	\end{tabular}
\end{table}

\honda{移植中}
The weights of terminal costs $S_{\mathrm{f}}$ are larger in order to reduce errors between terminal vehicle states and reference states. 
And, the weights of stage costs for state errors $Q$ are smaller so that the vehicle's states can be far away from reference states to avoid collision.
In addition, the weight of stage costs for the vehicle's acceleration $r^{\dot{v}}$ is larger in order to avoid sudden acceleration $\dot{v}$.
The weight for the vehicle's steering angle velocity $r^{\dot{\delta}}$ is smaller in order to greatly change its steering angle $\delta$ and yaw angle $\theta$ in tight space.
These weights need to be changed according to the purpose of the task. 


\honda{移植中}
We use IPOPT~\cite{IPOPT}, a solver based on the primal-dual interior method for solving the optimal control problem.
The primal-dual interior method is known as an algorithm that can solve large-scale non-linear programming problems with many inequality constraints quickly.
When a violation of constraints occurs, IPOPT searches for the solution in the direction of eliminating violations of constraints. 
At that time, IPOPT uses the gradients of constraint functions. 
Thus, we pay attention to the gradients of collision avoidance constraint functions.

\subsection{Evaluation Metrics}
To compare the calculation cost, we analyze the average and worst-case time of solving the optimal control problem at each time.
To compare the ability to navigate, we calculate the following indicator, success weighted by completion time(SCT) \cite{SCT}:
\begin{align}
	\mathrm{SCT}=\frac{1}{N}\sum_{i=1}^N S_i\frac{T_i}{\max(C_i,T_i)} \label{eq:SCT}
\end{align}
where $N$ is the number of episodes, $S_i$ takes 1 if the vehicle completes the episode $i$, otherwise it takes 0, $C_i$ is the vehicle's completion time, and $T_i$ is the vehicle's shortest completion time of all methods.
The more tasks are completed and the shorter the vehicle's completion time becomes, the higher SCT gets.
Then, SCT indicates the ability to navigate. 
The task is supposed to be completed when the vehicle's position is within a $0.2\ \mathrm{m}$ radius of the reference position and the vehicle's angle is within $\pm10\ \mathrm{degrees}$ from the reference angle.

\subsection{Simulation Results}

\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/reverse_parking/MSDE_path.pdf}
    \end{minipage}&
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/parallel_parking/MSDE_path.pdf}
    \end{minipage}\\
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/various_avoid/polygon.pdf}
    \end{minipage}&
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/various_avoid/circle.pdf}
    \end{minipage}
  \end{tabular}
  \caption{Trajectories with MSDE in reverse parking (Upper left), parallel parking (Upper right), avoidance of polygons (Lower left) and circles (Lower right).}
  \label{fig:trajectory}
\end{figure}
\begin{table}[t]
  \centering
	\footnotesize
  \caption{Simulation Results in the Parking Tasks}
  \label{tab:parking_sct}
	\begin{tabular}{|r|r|r|r|r|}\hline
		Parking type & \multicolumn{2}{c|}{reverse} & \multicolumn{2}{c|}{parallel} \\ \hline
		Method & SVM & MSDE & SVM & MSDE \\ 
		The number of variables & 523 & 145 & 397 & 145 \\ 
		SCT & 0.78 & 0.68 & 0.95 & 0.47 \\ \hline
	\end{tabular}
\end{table}
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/reverse_parking/ave_time.pdf}
    \end{minipage}&
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/reverse_parking/peak_time.pdf}
    \end{minipage}\\
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/parallel_parking/ave_time.pdf}
    \end{minipage}&
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{fig/parallel_parking/peak_time.pdf}
    \end{minipage}
  \end{tabular}
  \caption{Average and worst-case solving time in reverse parking (Upper row) and parallel parking (Lower row).}
  \label{fig:solving_time}
\end{figure}

\figref{fig:trajectory} shows 4 examples of scenarios with MSDE.
In reverse and parallel parking, the vehicle went back and forth while cutting the wheel repeatedly and succeeded in parking without collisions by both methods.
\figref{fig:solving_time} shows box plots of average and worst-case solving time in reverse and parallel parking with two methods, respectively.
MSDE's solving time was much lower than SVM's.
On the one hand, SVM's constraint function $q_i(ax_i+by_i+c)$ is bilinear.
Thus, both changes of two variables in the first and second terms of the function need to be considered at once.
On the other hand, MSDE's constraint function $d_j$ is linear when the obstacle is static.
With algorithmic differentiation of the minimum function, the minimum argument is differentiated \cite{algorithmic_differentiation}.
Hence, MSDE's constraint function $d_j$ is treated as a linear function.
Roughly speaking, while SVM needs to optimize both separate lines' movements and the vehicle's one, MSDE only needs to optimize the latter.
Moreover, SVM needs more decision variables than MSDE by parameters of separate lines. 
That's why the calculation cost of MSDE was lower than that of SVM.
\tabref{tab:parking_sct} shows SCT and the number of decision variables of two methods in reverse and parallel parking.
SVM's SCT was higher than MSDE's.
The number of decision variables is larger with SVM than with MSDE, so the searching range for the solution is also larger with SVM.
Thus, SVM could find a better solution that MSDE could not find.
On the one hand, the gradient of MSDE's constraint function $d_j$ changes discontinuously when its minimum argument $l_i(x,y)$ switches.
On the other hand, SVM's constraint function $q_i(ax_i+by_i+c)$ does not contain any minimum functions, so its gradient is continuous in all fields.
Therefore, SVM can numerically eliminate the violation of constraints more easily than MSDE. 
That's why SVM's ability to navigate was higher than MSDE's.

In avoidance of polygons and circles, the vehicle reached its destinations without collisions with both methods, as shown in \figref{fig:trajectory}. And, its completion time is the same between the two methods.
\tabref{tab:various_avoid_sct} shows the number of decision variables, the average and worst-case solving time of the two methods in the avoidance of polygons and circles.
MSDE's average and worst-case solving time is much shorter than SVM's.
The results about solving time are the same as those in parking simulations, so the reason should also be the same. 

\begin{table}[t]
  \centering
	\footnotesize
  \caption{Computational Cost}
  \label{tab:various_avoid_sct}
	\begin{tabular}{|r|r|r|r|r|}\hline
		Obstacle & \multicolumn{2}{c|}{polygons} & \multicolumn{2}{c|}{circles} \\ \hline
		Method & SVM & MSDE & SVM & MSDE \\ 
		The number of variables & 271 & 145 & 586 & 145 \\ 
		Average solving time [ms]& 100 & 54.0 & 622 & 123 \\
        Worst-case solving time [ms]& 511 & 224 & 17901 & 650 \\ \hline
	\end{tabular}
\end{table}

\subsection{Real World Experiment Settings}

To experimentally compare the two avoidance methods in the real world, a \textit{LIMO Pro} is used.
The \textit{LIMO Pro} is a small steering vehicle which can be programmed using ROS.
Its length $l_{\mathrm{car}}$ is $322\ \mathrm{mm}$, width $w_{\mathrm{car}}$ is $220\ \mathrm{mm}$, wheMSDEbase $l_{\mathrm{f}}$ is $200\ \mathrm{mm}$, and rear overhang $l_{\mathrm{roh}}$ is $70\ \mathrm{mm}$.
We set the \textit{LIMO Pro}'s margin  $d_{\mathrm{margin}}=20\ \mathrm{mm}$, absolute limit of velocity $v_{\mathrm{lim}}=2\ \mathrm{m/s}$, steering angle $\delta_{\mathrm{lim}}=0.35\ \mathrm{rad}$, accMSDEeration $\dot{v}_{\mathrm{lim}}=1\ \mathrm{m/s^2}$ and steering angle velocity $\dot{\delta}_{\mathrm{lim}}=6.28\ \mathrm{rad/s}$.
The \textit{LIMO Pro} accepts control inputs as the velocity and steering angle, so their solution of the optimal control problem is used as control inputs.
4 RC cars are parked before the \textit{LIMO Pro} parks, and their positions are supposed to be known.
To park among them, the following control cycle is applied.
The \textit{LIMO Pro}'s position and yaw angle are observed by motion capture and sent to a notebook.
Motion capture uses 10 ceiling cameras and 9 markers on the roof of the \textit{LIMO Pro}, and its sampling frequency is $100\ \mathrm{Hz}$.
The notebook is the same as the one used in simulations.
The observed \textit{LIMO Pro}'s position and yaw angle are used as its initial states of the optimal control problem.
Then, the problem is solved in the notebook, and the obtained control inputs for the first step future are sent to the \textit{LIMO Pro}.
This cycle is repeated until the \textit{LIMO Pro} reaches the parking spot.

\subsection{Real World Experiment Results}

\figref{fig:experiment_solving_time} shows solving time for each MPC cycle in experiments with SVM and MSDE.
On the one hand, SVM's average and worst-case solving time were $3.19\ \mathrm{s}, 97.8\ \mathrm{s}$, respectively. 
Hence, its solving time was often over the time interval of the prediction horizon $\Delta\tau=0.2\ \mathrm{s}$.
Thus, the \textit{LIMO Pro} got out of control, collided with some RC cars and could not park among RC cars. 
On the other hand, MSDE's average and worst-case solving time were $139\ \mathrm{ms}, 689\ \mathrm{ms}$, respectively.
Then, its solving time was often within the time interval of the prediction horizon.
Therefore, the \textit{LIMO Pro} smoothly parked among RC cars without any collisions, as shown in \figref{fig:experiment_path}. 
In addition, it went back and forth only once, and its completion time was relatively short, $17.3\ \mathrm{s}$.
\figref{fig:experiment_control_input} shows control inputs applied to the \textit{LIMO Pro} in the experiment with MSDE. 
According to weights' settings in \secref{sec:evaluate_function}, it accelerated smoothly, and its steering angle greatly changed.
Comparing experiment results with two methods,
it will be important for controlling the vehicle in real time to reduce the calculation cost rather than to improve the ability to navigate it.

\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=6cm]{fig/experiment/limo_SVM_ts.pdf}
    \end{minipage}\\
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=6cm]{fig/experiment/limo_MSDE_ts.pdf}
    \end{minipage}
  \end{tabular}
  \caption{Solving time for each MPC cycle in real-world experiments with our proposed methods, SVM(Above) and MSDE(Below). Be careful of their different scales.}
  \label{fig:experiment_solving_time}
\end{figure}

\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=7cm]{fig/experiment/robot_motion_overlay.png}
    \end{minipage}\\
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=7cm]{fig/experiment/limo_MSDE_path.pdf}
    \end{minipage}
  \end{tabular}
  \caption{A real-world experiment result with our proposed method (MSDE). }
  \label{fig:experiment_path}
\end{figure}

\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=6cm]{fig/experiment/limo_v.pdf}
    \end{minipage}\\
    \begin{minipage}[t]{0.45\hsize}
      \centering
      \includegraphics[width=6cm]{fig/experiment/limo_delta.pdf}
    \end{minipage}
  \end{tabular}
  \caption{Velocity and steering angle applied to \textit{LIMO Pro} in a real-world experiment with our proposed methos (MSDE).}
  \label{fig:experiment_control_input}
\end{figure}

